The Efficiency Spectrum of Large Language Models: An Algorithmic Survey

The rapid growth of Large Language Models (LLMs) has been a driving force in transforming various domains, reshaping the artificial general intelligence landscape. However, the increasing computational and memory demands of these models present substantial challenges, hindering both academic research and practical applications. To address these issues, a wide array of methods, including both algorithmic and hardware solutions, have been developed to enhance the efficiency of LLMs. This survey delivers a comprehensive review of algorithmic advancements aimed at improving LLM efficiency. Unlike other surveys that typically focus on specific areas such as training or model compression, this paper examines the multi-faceted dimensions of efficiency essential for the end-to-end algorithmic development of LLMs. Specifically, it covers various topics related to efficiency, including scaling laws, data utilization, architectural innovations, training and tuning strategies, and inference techniques. This paper aims to serve as a valuable resource for researchers and practitioners, laying the groundwork for future innovations in this critical research area. Our repository of relevant references is maintained at url{https://github.com/tding1/Efficient-LLM-Survey}.

==> 07-infrastructure.tex <==
\section{Infrastructure Efficiency}\label{sec:infrastructure}

The above breakthroughs of algorithmic designs high relies on the development of underlying infrastructures including both software and hardware. We will describe up-to-date infrastructure achievement in this section. 

\subsection{Introduction} The fundamental AI infrastructure for efficient LLM can be largely categorized into two aspects, \emph{i.e.,} software and hardware. The software 

\subsection{Software}

\td{Starting point: \cite[Sec 3.3]{zhao2023survey}}

\paratitle{DeepSpeed}~\cite{rasley2020deepspeed} is a deep learning optimization library designed to make distributed training more efficient and easy to use. Developed by Microsoft, the library aims to help researchers and engineers train massive models with minimal code changes, allowing for faster experimentation. DeepSpeed offers several key optimizations for improving the speed and resource efficiency of deep learning models, including, (i) Memory Efficiency: Techniques like memory-efficient optimizer state, and ZeRO (Zero Redundancy Optimizer) stages 1, 2, and 3, to allow for model training with less GPU memory, (ii) Model Parallelism: Enables the training of models that are too large to fit into a single GPU by partitioning them across multiple GPUs. (iii) Data Parallelism: Efficiently scales out the training process across multiple GPUs and even nodes. (iv) Pipeline Parallelism: For extremely large models, DeepSpeed can parallelize the model across multiple stages, which can then be executed in a pipelined fashion across multiple GPUs. By integrating DeepSpeed into existing deep learning frameworks like PyTorch, researchers and engineers can utilize these and other optimizations to accelerate their work. It aims to make it easier to train models that are both bigger and faster, while also allowing for more efficient use of hardware resources.

\paratitle{Megatron-LM}~\cite{shoeybi2019megatron, narayanan2021efficient} is a model-parallelism library developed by NVIDIA. It is designed to scale up the training of large machine learning models across multiple GPUs. Megatron is particularly useful for training enormous transformer-based models, including the GPT (Generative Pre-trained Transformer) and BERT (Bidirectional Encoder Representations from Transformers) architectures.

The primary purpose of Megatron is to facilitate the training of models that are too large to fit into the memory of a single GPU. By using model parallelism, Megatron divides the model into smaller pieces via tensor parallelism, distributing them across multiple GPUs for training. This enables researchers and developers to train substantially larger models than they otherwise could, potentially leading to better performance and capabilities.

Megatron has been used in the development of some of the largest language models to date, and it complements data parallelism techniques to maximize hardware utilization further. It's part of a broader ecosystem of tools and libraries aimed at making large-scale machine learning more accessible and efficient.

\paratitle{Colossal-AI}~\cite{li2021colossal}  Data, Model, Pipeline Parallelism

\paratitle{BMTrain}~\cite{BMTrain}  \url{}

\paratitle{FastMoE}~\cite{he2021fastmoe}

\paratitle{LLaMaCPP}~\cite{llamacpp}

\paratitle{RWKV-LM}~\cite{peng2023rwkv}

\subsection{Hardware}

\td{Starting point: \cite[Sec 4]{zhuang2023survey}}

MLC-LLM~\cite{mlcllm}

NVIDIA Semi-Structured Sparsity A100

\subsection{Summary}

==> 08-discussion.tex <==
\section{Future Directions and Open Challenges}\label{sec:discussion}

\subsection{Summary of scaling law.}
The ability to generalize how performance scales with model size, dataset size, and computation budget, as estimated from small-scale cases, provides valuable guidance for scaling these factors and predicting performance before training large language models. Many other factors, such as data quality and model architectures, could also significantly impact the scaling behavior. We will review recent developments in data selection and architectures in the following sections.


\subsection{Summary of efficient architecture}
As the computation of attention is still dominating the overall cost of the Transformer architecture~\cite{vaswani2017attention}, the directions mentioned above are mostly focusing on how to reduce such time cost (efficient attention, efficient positional encoding or attention free architectures instead of self-attention) or improving the performance without further increasing the time needed for the pipeline (sparse modelling). The former one focuses on reducing the required computation by reducing the sparsity in the model while, interestingly, the latter one is trying to make use of the sparsity and activate only parts of them during the feedforwarding process with more expertise branches. Although treating the sparsity in different manners, they have reached the same destination, which is to have a more efficient pipeline compared to the original large models, without compromising their performance or even improve it.

\subsection{Summary of training and tuning}

This work \cite{chen2022revisiting} demonstrates that parameter-efficient tuning methods (i) can exhibit instability across different random seeds and (ii) yield varying performance across different tasks and settings, such as the number of training samples and tunable parameters. These methods often achieve comparable performance for low-resource tasks but inferior performance for medium to high-resource tasks when compared to full fine-tuning.
